Two-shot Video Object Segmentation

Previous works on video object segmentation (VOS) are trained on densely annotated videos. Nevertheless, acquiring annotations in pixel level is expensive and time-consuming. In this work, we demonstrate the feasibility of training a satisfactory VOS model on sparsely annotated videos-we merely require two labeled frames per training video while the performance is sustained. We term this novel training paradigm as two-shot video object segmentation, or two-shot VOS for short. The underlying idea is to generate pseudo labels for unlabeled frames during training and to optimize the model on the combination of labeled and pseudo-labeled data. Our approach is extremely simple and can be applied to a majority of existing frameworks. We first pre-train a VOS model on sparsely annotated videos in a semi-supervised manner, with the first frame always being a labeled one. Then, we adopt the pre-trained VOS model to generate pseudo labels for all unlabeled frames, which are subsequently stored in a pseudo-label bank. Finally, we retrain a VOS model on both labeled and pseudo-labeled data without any restrictions on the first frame. For the first time, we present a general way to train VOS models on two-shot VOS datasets. By using 7.3% and 2.9% labeled data of YouTube-VOS and DAVIS benchmarks, our approach achieves comparable results in contrast to the counterparts trained on fully labeled set. Code and models are available at https://github.com/yk-pku/Two-shot-Video-Object-Segmentation.

==> figures/bidirectional.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\columnwidth]{./imgs/bidirectional.pdf}
  \caption{Illustration of unidirectional inference \textit{vs}. bidirectional inference. It is obvious that using labeled frame $15$ to infer unlabeled frame $105$ lead to poor mask prediction due to the accumulation error of feature propagation. Instead, using labeled frame $110$ to infer unlabeled frame $105$ in a reverse direction can obtain better results, which is more suitable for initializing the label bank.}
  \label{fig:bidirectional}
\end{figure}
